Syntactic Abstraction of B Models to Generate Tests

In a model-based testing approach as well as for the verification of properties, B models provide an interesting solution. However, for industrial applications, the size of their state space often makes them hard to handle. To reduce the amount of states, an abstraction function can be used, often combining state variable elimination and domain abstractions of the remaining variables. This paper complements previous results, based on domain abstraction for test generation, by adding a preliminary syntactic abstraction phase, based on variable elimination. We define a syntactic transformation that suppresses some variables from a B event model, in addition to a method that chooses relevant variables according to a test purpose. We propose two methods to compute an abstraction A of an initial model M. The first one computes A as a simulation of M, and the second one computes A as a bisimulation of M. The abstraction process produces a finite state system. We apply this abstraction computation to a Model Based Testing process.

==> 20100120_CR.tex <==

Modifs pour garder ModX + syntaxique de abstract varialbes
  * 


Actions : 
  PAM propose de fusionner sections 5 et 6 en les orientant application.
  MàJ de l'introduction et conclusion
  Section 2 : retirer les substitution verbeuse mais garde @x(P=>S) & IF
              remplacer def de Prd par sa def générale

  Quid du raffinement ? L'introduire en section 4 ? Le mettre en annexe ? Laisser en 2 ? 

  Rajouter quelques phrases d'intuition pour alléger la lecture
  Attention au mot clef "substitution" qui peut être lourd.

  Section 3 : Corriger le footnote pour l'explication de la restriction du co-domaine
               --> mettre en une phrase plutôt qu'en footnote

  section 4 : 
     Section 4.1 : parler de control / data flow plutôt que syntaxique / sémantique
                   introduire data flow avant les 2 
                   Sur/sous approximation : ne pas dire ça. Parler plutôt de la taille de l'ensemble des variables abstraites.
                   Dans la def de ModX, les i en indice sont inutiles.
                   Retirer la ligne "If prime variables was being ..... "
                   Retirer la table 1 et corriger/relire la table 2 
                   Prendre le cas général de @ dans la table 2
                   Commenter 2-3 règles de ModX pour donner une bonne intuition


   section 4.5 : 
      faire une intro
      garder 2 preuves et théorème en fonction du choix des variables.
      Laisser les preuves en annexe
      Ajouter le lien entre Prd et événement à travers la forme normale ?

   Section 7 : 
      Commencer par expliquer méthode utiliser pour le choix des variables pour chaque exemple.
      Attention aux infos 'int' pour le modèle du syst électrique

Réfléchir à ce qui serait impacter si un passer sur un modèle à états infini (nb batteries non défini, ou avec une constante)



TODO : 
  fusion sections 5 et 6 : PAM
  retouches section 2    : JJ
  retouches section 4.1  : NS suivi par JJ 
  retouches section 4.5  : JJ
  reformuler annexe      : NS (dans le sens du prd)

  Réfléchir à ce qui serait impacter si un passer sur un modèle à états infini (nb batteries non défini, ou avec une constante)

 

Déporté à plus tard :
  MàJ de l'introduction et conclusion
  



==> sec5bis-genTestsFromAbs.tex <==
%%%% MACROS
\newcommand{\SD}{\textsf{SD}\xspace} % SDO + complement
\newcommand{\genesyst}{\textsf{Genesyst}\xspace}
\newcommand{\SP}{\textsf{SP}\xspace} % Synchrous Product
\newcommand{\AST}{\textsf{AST}\xspace} % {abstract symbolic tests}
\newcommand{\CL}{\textsf{CL}\xspace} % {concretization layer}
\newcommand{\IT}{\textsf{IT}\xspace} % {instantiated tests}




\section{Test Generation Process from Dynamic Selection Criteria and
Abstractions}
\label{sec:process-test}
Let us present our motivations, and our process for generating tests
from dynamic selection criteria and abstractions.


%---------------------------------------
\subsection{Problem and Motivations}
\label{subsec:problematics}
In our approach, the validation engineer describes by means of an
hand-written test purpose \tp how he intends to test the system,
according to his know-how.  We have proposed in~\cite{jmt-ast08-langage} a
language based on regular expressions, to describe a \tp as a sequence
of actions to fire and states to reach (targeted by these actions).
The states are described as state predicates. The actions can be
explicitely called by their name, or left unspecified by the use of a
generic name.  This genericity allows the tester to describe a
situation to reach without specifying \emph{how} it should be reached.
But a regular expression repetition operator can be applied to the
unspecified action call.  This means in the tester's mind: leaving all
possibilities to the system to reach a target state. The drawback is a
combinatorial explosion of the number of executions of \fm in which to
search for an instantiation of the action calls that reach the target
state. The search should be guided to avoid that problem.

% But the drawback is a potential
% combinatorial explosion of the number of executions of \fm described by
% such a \tp.
% in which to search for an instantiation reaching that target state.
%
%
% In~\cite{fac09}, we have presented a test generation approach from a
% \tp and a \B model \fm, that proceeds by unfolding all the paths of the
% automaton associated to the \tp.  Each path is a symbolic test, in the
% sense that the values of the action parameters are not defined. They
% will be defined by an instantiation phase, that
% % uses
% applies to \fm
% %
% constraint solving techniques and data boundary valuation strategies.
% Also, the test must be concretized to become executable on the IUT.
% This approach has been successfully experimented on an industrial
% application such as IAS~\cite{Gix04},
%%% nEW
% but with a limited use of the genericity of the language.
%% OLD
% Nevertheless, two points need to be improved in the method.
%
%%% NEW
% Indeed, a regular expression repetition operator such as * or + can be
% applied to the unspecified action call \dollarop. This means in the
% tester's mind: leaving all possibilities to the system to reach a
% target state. 

% But the result is a combinatorial explosion of the
% number of executions of \fm in which to search for an instantiation
% reaching that target state. The search should be guided to avoid that
% problem.





\subsection{Test Generation Process by Abstraction}
%---------------------------------------------------
A small size state-transition graph, that symbolically models the
executions of the system, can be obtained by computing an abstraction
\abs of \fm.  
%
We propose to perform a synchronized product between \abs and
the automaton of the \tp,  
% : this is easy due to the small size of \abs.
and to use paths of the synchronized product as guides for the
instantiation of the \tp on \fm.


 
% This abstraction brings
% answers to the aforementioned two points. The first point is addressed
% by generating the tests from the synchronized product of the
% abstraction \abs with \tp. These symbolic \emph{abstract} tests are more
% precise than the ones obtained with the~\cite{fac09} approach.  The
% abstraction has brought the activation conditions of the actions in
% the shape of a conjunction of a predicate that defines the symbolic
% state and a guard enabling the transition.
% The abstraction has also instantiated all the generic action names
% of the \tp with a subset of the actions of the model \fm. As for the
% second point, the measure of the coverage achieved by a test suite is
% now performed on the synchronization \SP of \abs and \tp. This is
% much more relevant as the coverage is measured w.r.t. the executions
% of \fm that satisfy \tp and not only w.r.t. \tp.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%--------
\begin{figure}[th]
\begin{center}
\includegraphics[scale=0.35]{procITfromAbs.eps} 
\caption{Generating Tests from Test Purpose by Abstraction}
\label{fig:genTestByAbs}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%--------


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%--------
% \begin{figure*}[th]
% % \begin{center}
% \centering
% \begin{tabular}{cc}
% \includegraphics[scale=0.3]{procMBTabs.eps} & 
% \includegraphics[scale=0.3]{procMBTdyn.eps}  \\
% (a) MBT from an abstraction & (b) MBT with dynamic criterion  \\
% \multicolumn{2}{c}{\includegraphics[scale=0.3]{procMBTstatic.eps}}  \\
% \multicolumn{2}{c}{(c) MBT with static criterion}   \\
% \end{tabular}
% \caption{Generating tests by abstraction}
% \label{fig:genTestByAbs}
% % \end{center}
% \end{figure*}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%--------
Our approach is depicted in Fig.~\ref{fig:genTestByAbs}. 
% From a behavioral model \fm and the state variables of a \tp, we
% define a set \SD of abstraction predicates. \SD stands for sub-domains
% (of the state variables). The details of this definition can be found
% in~\cite{bbjm-amost10}. The \genesyst tool~\cite{genesystZB05} produces an
% abstraction \abs of \fm based on the predicates of \SD.
The synchronized product of \abs with the \tp results in a model \SP.
The executions of \SP are the executions of \abs that match the
\tp. An implementation~\cite{Thi03} of the Chinese Postman algorithm
is applied to \SP to cover its transitions. The result is a set of
abstract symbolic tests \AST. These tests are instantiated from \fm.
% ,
% which allows for re-using the same test execution environment
% (i.e. the concretization layer \CL and the test execution tools) as of
% Fig.~\ref{fig:standardMBT}: the new instantiated tests \IT (of
% Fig.~\ref{fig:genTestByAbs}) complement the ones of
% Fig.~\ref{fig:standardMBT}. 
%
Notice the dashed arrow in
Fig.~\ref{fig:genTestByAbs} from \SP to the ``instantiation''
box. This is because, to instantiate the abstract symbolic tests, we
use the reflexive transitions of \SP that were ignored to generate
\AST.  % This point is explained in Sec.~\ref{subsec:testInstantiation}.


%%% OLD Comments with regards to the old figure in 3 views
% View~\ref{fig:genTestByAbs}(c) shows the
% usual MBT process with static (control and data) selection criteria. The MBT
% process with dynamic criteria is obtained by replacing the input \fm of
% View~\ref{fig:genTestByAbs}(c) by the output \SP
%  of View~\ref{fig:genTestByAbs}(b). The
% process that we propose combines the three views by replacing the
% input \fm of View~\ref{fig:genTestByAbs}(b) with the output \abs of
% View~\ref{fig:genTestByAbs}(a). The effect is to replace the detailed
% model \fm, input of the MBT process, with an abstraction of \fm.
% \begin{itemize}
% \item \textbf{View~\ref{fig:genTestByAbs}(c).} From a behavioral
%   model \fm written by the validation engineer and from static 
%   selection criteria on the control structures of the model,
%   % (such as \emph{all the states}, or \emph{all the transitions}),
%   the test generation tool (LTG in our case) computes a set of
%   abstract tests \AT. The instantiation computes parameter values for
%   the action calls, providing a set of instantiated tests \IT. This
%   relies on data selection criteria such as boundary valuation
%   strategies. These tests are still as abstract as \fm and must be
%   concretized \emph{via} a concretization layer \CL into a set of
%   concrete tests \CT, that are executed on the \IUT. This delivers a
%   verdict of success or failure, by comparing the results predicted by
%   \fm with the ones returned by the \IUT.

% \item \textbf{View~\ref{fig:genTestByAbs}(b).} The input \fm in
%   View~\ref{fig:genTestByAbs}(c) is replaced with a model \SP,
%   that results from the synchronization of \fm with a dynamic selection
%   criteria \tp. Thus the executions of \SP are the executions of
%   \fm that match \tp.

% \item \textbf{View~\ref{fig:genTestByAbs}(a).} There again, the
%   input \fm of the previous process (View~\ref{fig:genTestByAbs}(b)),
%   is replaced with another input: an abstraction \abs of the model
%   \fm. The originality of our approach comes from the fact that this
%   abstraction is \emph{computed} from \fm and a \tp, and not directly
%   given by the validation engineer. The abstraction is computed in two
%   steps: $(i)$~a set \SS of symbolic states of the abstraction is
%   computed from the information in \tp (see
%   Sec.~\ref{subsec:defOfSymbStates}). The aim is to observe \fm
%   w.r.t. this information; $(ii)$~an abstraction \abs is
%   computed. Its symbolic states are the ones defined by \SS. In
%   practice, as the model \fm is defined in \textsf{B}, we use
%   \genesyst~\cite{genesystZB05} to compute the abstraction.
% %  We define for
% %   this tool the set of symbolic states \SS as an assertion that is a
% %   disjunction of predicates. Each predicate defines a symbolic state.
% \end{itemize}



